QRFA: A Data-Driven Model of Information-Seeking Dialogues

Understanding the structure of interaction processes helps us to improve information-seeking dialogue systems. Analyzing an interaction process boils down to discovering patterns in sequences of alternating utterances exchanged between a user and an agent. Process mining techniques have been successfully applied to analyze structured event logs, discovering the underlying process models or evaluating whether the observed behavior is in conformance with the known process. In this paper, we apply process mining techniques to discover patterns in conversational transcripts and extract a new model of information-seeking dialogues, QRFA, for Query, Request, Feedback, Answer. Our results are grounded in an empirical evaluation across multiple conversational datasets from different domains, which was never attempted before. We show that the QRFA model better reflects conversation flows observed in real information-seeking conversations than models proposed previously. Moreover, QRFA allows us to identify malfunctioning in dialogue system transcripts as deviations from the expected conversation flow described by the model via conformance analysis.

==> addon/commands.tex <==
\RequirePackage{rotating}

\newcommand{\sidewaysheader}[1]{\begin{sideways}{#1}\end{sideways}}
\newcommand{\sidewaysheaderpar}[2]{\begin{sideways}\parbox{#1}{\centering #2}\end{sideways}}

\RequirePackage{paralist}
\newenvironment{iiilist}%
{\begin{inparaenum}[\itshape(i)\upshape]}%
{\end{inparaenum}}

\RequirePackage{colortbl}

\newcommand{\grayrow}{\rowcolor{gray!20}} %
\newcommand{\lightgrayrow}{\rowcolor{gray!10}} %
\newcommand{\graycell}{\cellcolor{gray!30}} %

% To color text
\RequirePackage{xcolor}
% To create side-notes
\RequirePackage{marginnote}
%
\newenvironment{AuthNote}[1][]{%
    \ifx\newenvironment#1%
      \newenvironment%
    \else%
      \marginnote{\scriptsize{Note: #1}}%
    \fi%% Write a margin note with a title, if provided
    \begin{scriptsize}%% Change the default size of the font
    \colorbox{gray}%
    {\color{white} Note: }%
    \quad%
    \color{brown}%% Change the colour to brown
%    \ifx\newenvironment#1\newenvironment\marginnote{\scriptsize{Notes}}\else\marginnote{\scriptsize{Note: #1}}\fi%% Write a margin note, optionally with a title
  }{%
    \normalcolor%% Restore the normal colour
    \end{scriptsize}%% Restore the normal size
}

% Alter the margin paragraph width
%\marginparwidth=2.5cm

%% Subsubsection without waste of space
\newcommand{\mysubsubsection}[1]{\noindent\textbf{#1}}

==> addon/glossary.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Acronyms / abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\newacronym[\glslongpluralkey={Business Processes}]{bp}{BP}{Business Process}
\newacronym{bpi}{BPI}{Business Process Intelligence}
\newacronym{bpm}{BPM}{Business Process Management}
\newacronym{bpmn}{BPMN}{Business Process Model and Notation}
\newacronym{bpms}{BPMS}{Business Process Management System}
\newacronym{kpi}{KPI}{Key Performance Indicator}
\newacronym{ppi}{PPI}{Process Performance Indicator}
\newacronym{soa}{SOA}{Service-Oriented Architecture}
\newacronym{wf}{WF}{workflow}
\newacronym{wfms}{WfMS}{Workflow Management System}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keywords
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Log, trace, event --------------------------------------------
%
% log alphabet
\def\LogAlph {\ensuremath{\mathcal{A}}}
\newglossaryentry{logalph}{
	name={log alphabet},description={process alphabet, as reflected in the log},%
	symbol={\LogAlph}}
%
% event
\def\Evt {\ensuremath{e}}
\newglossaryentry{evt}{
	name={event},description={a record of an instantaneous fact during the process enactment},%
	symbol={\Evt}}
%
% trace
\def\Trace {\ensuremath{t}}
\newglossaryentry{evttrace}{
	name={trace},description={a sequence of \glsentrytext{event}s},%
	symbol={\Trace}}
%
% event log
\def\EvtLog {\ensuremath{L}}
\newglossaryentry{evtlog}{
	name={event log},description={a collection of \glsentrytext{trace}s},%
	symbol={\EvtLog}}
%
% task
\newglossaryentry{task}{%
	name={task},description={The non-divisible, elementary activity}}

==> addon/memorandum.tex <==
% !TeX root = ../main.tex
%
\section*{For us authors: some tips and tricks}
\label{sec:memo}
%%%
%%% Start of: preliminary commands to be used exclusively in this file.
%%%
\newglossaryentry{test}{name={test},description={A fictionary test}}
\newacronym{testacro}{TA}{Test Acronym}
%%%
%%% End of: preliminary commands to be used exclusively in this file.
%%%
%
% --------------------------------
% About comments
% --------------------------------
%
\hl{For your comments}, please use the
\todo[inline]{\texttt{todo} environment, either in-line or }
or aside.
\todo{aside}
%
You can even add missing figures with the \verb|\missingfigure| command (see \cref{fig:example:missing:figure}).
\begin{figure}[b]
\missingfigure{\texttt{{\textbackslash}missingfigure} command}
\caption{A missing figure}
\label{fig:example:missing:figure}
\end{figure}
%
\\
%
% --------------------------------
% About inline lists
% --------------------------------
%
\hl{For lowercase-roman-enumerated inline lists}, please use
\begin{iiilist}
\item the
\item \texttt{iiilist}
\item environment.
\end{iiilist}
It is a custom command you find in \verb|addons/commands.tex|. It is based on the \verb|\inparaenum| command, from package \textit{paralist}.
%
\\
%
% --------------------------------
% About keywords
% --------------------------------
%
\hl{For specific terms}, which may change in the future, add a \hl{glossary} entry in \texttt{addons/glossary.tex},
and use
\begin{iiilist}
\item the \texttt{gls} command to use them (e.g., \gls{test}),
\item the \texttt{Gls} command for capitalising them (e.g., \Gls{test}),
\item the \texttt{glspl} command for obtaining their plural form (e.g., \glspl{test}), and
\item the \texttt{Glspl} command for for obtaining their plural capitalised form (e.g., \Glspl{test}).
\end{iiilist}
It turns out to be very useful in those situations in which the co-authors do not remember, for example, whether they should indicate the sequences of executed actions as ``traces'' or ``runs''. To solve the issue and avoid that all co-authors write different things, they can decide on a temporary solution (say, ``traces''), make it a glossary entry (say, \verb+\newglossaryentry{actx}{name={trace},description={...}}+), use \verb+\gls{actx}+ (or similar commands -- see above) every time they want to say that thing, and when the opinion on the best term will change (in favour of ``runs''), it will be enough to change the glossary entry definition (\verb+\newglossaryentry{actxeq}{name={run},description={...}}+) and see it varied everywhere it was used in the text. Another use case is: ``AB Testing'' or ``AB testing''? To avoid that the ``T''s of ``testing'' occur as upper-case sometimes, and as lower-case at times, a single glossary entry comes handy!
%
\\
%
\hl{For acronyms}, they are meant be defined within the same file as follows: \texttt{{\textbackslash}newacronym\{testacro\}\{TA\}\{Test Acronym\}}.
They can be referenced by using \texttt{{\textbackslash}Gls} (plus variants for plural forms etc.).
Result is, you get the full version the first time the acronym is used
-- \texttt{{\textbackslash}gls\{testacro\}} is displayed as \Gls{testacro}.
From the second time onwards, the call will return the acronym only, without any description:
\texttt{{\textbackslash}gls\{testacro\}} is displayed as \Gls{testacro}.
To force the representation to have either long or short versions, use
\texttt{{\textbackslash}acrlong\{testacro\}}
(leading to \acrlong{testacro})
or
\texttt{{\textbackslash}acrshort\{testacro\}}
(displaying \acrshort{testacro}).
Acronyms are collected in \texttt{addons/glossary.tex} too.
%
\\
%
\hl{To refer to sections, tables, figures, etc.}, please use the \texttt{cref} command (e.g., \cref{sec:memo}).
\texttt{Cref} capitalises and expands the specifier of the referred document part (e.g., \Cref{fig:example:missing:figure}). It is best to be used at the beginning of phrases, whereas \texttt{cref} uses the abbreviation (e.g., \cref{fig:example:missing:figure}).
%

==> addon/pkgloading.tex <==
% For language-specific hyphenations etc.
\usepackage[english]{babel}
% For subfigures
\usepackage{subcaption}
% For nice links
\usepackage{url}
% For playing with colors in tabular environments
\usepackage{colortbl}
% For math symbols, such as \nexists
\usepackage{amssymb}
% For more math symbols, such as \mapsfrom
\usepackage{stmaryrd}
% For advanced graphics
%% For including figures, graphicx.sty has been loaded in
%% elsarticle.cls. If you prefer to use the old commands
%% please give \usepackage{epsfig}
% For equations, arrays of equations, defining operator names, etc.
\usepackage{amsmath}
% For cursive math
\usepackage{mathrsfs}
% For math symbols, such as \nexists
\usepackage{amssymb}
%% For math environments, such as "definition"
%\usepackage{amsthm}
%\theoremstyle{definition}
%\newdefinition{definition}{Definition}[section]
%\newtheorem{theorem}{Theorem}[section]
% For enumerating the line numbers
\usepackage[left]{lineno}
% For side notes, missing figures and inline to-do's
\usepackage[textsize=scriptsize,backgroundcolor=yellow!40]{todonotes}
% For specifying kewords and acronyms
\usepackage[nonumberlist,acronym,sanitize=none]{glossaries}
\glsdisablehyper
% For commenting out some parts of the text
\usepackage{comment}
% For building hyperlinks
\usepackage[pdftex, colorlinks=true, hyperfootnotes=true, hyperindex=true,
            plainpages=false, pagebackref=false, pdfpagelabels=true, pdfstartview=FitH,
            linkcolor=blue, citecolor=blue, urlcolor=blue,
            bookmarks, bookmarksopen, bookmarksdepth=3]{hyperref}
% For smart references
\usepackage[capitalise,nameinlink]{cleveref}
% To have "Figure 3(a)" in place of "Figure 3a" and  "Table 3(a)" in place of "Table 3a"
\captionsetup[subfigure]{subrefformat=simple,labelformat=simple}
    \renewcommand\thesubfigure{(\alph{subfigure})}
\captionsetup[subtable]{subrefformat=simple,labelformat=simple}
    \renewcommand\thesubtable{(\alph{subtable})}
\Crefname{algocf}{Algorithm}{Algorithms}
% TikZ/Pgf advanced graphics
\usepackage{tkz-base}
\usetikzlibrary{decorations.pathmorphing,trees,snakes,arrows,shapes,automata}
% To use inline and other fancy list-like environments (e.g., inparaenum)
\usepackage{paralist}
% To divide a text line into multiple columns
\usepackage{multicol}
% To create good-looking book-style tables
\usepackage{booktabs}
% To play around with list environments
\usepackage{enumitem}
% To create multirow cells in tables
\usepackage{multirow}
% To create rotated cells in tables
\usepackage{rotating}
% To create enumerated lists, whose numbering is reversed
\usepackage{etaremune}
%% To make algorithmic nice-looking pseudocode
% \usepackage[ruled,linesnumbered,algo2e]{algorithm2e}
%% For creating side-notes
% \usepackage{marginnote}
% For superimposing symbols over one another within math env.
\usepackage{mathtools}
% For strange math symbols like \Dashv
\usepackage{mathabx}
% For LaTeX if/then statements
\usepackage{ifthen}
% For strike-through cancellations
\usepackage[normalem]{ulem}
%% The lineno packages adds line numbers. Start line numbering with
%% \begin{linenumbers}, end it with \end{linenumbers}. Or switch it on
%% for the whole article with \linenumbers.
\usepackage{lineno}
% For highlighted text
\usepackage{soul}
% To put table environments and co. side by side
\usepackage{floatrow}
\floatsetup[table]{style=plaintop}
% To add dummy text
\usepackage{lipsum}
% To have newlines in cells, with commands such as \makecell or \thead
\usepackage{makecell}
% For a decent formatting of numbers (and a wonderful system for numeric columns in tables, ``S'')
\usepackage{siunitx}
% To enable text protrusion
\usepackage{microtype}

